Neural-FST Class Language Model for End-to-End Speech Recognition

We propose Neural-FST Class Language Model (NFCLM) for end-to-end speech recognition, a novel method that combines neural network language models (NNLMs) and finite state transducers (FSTs) in a mathematically consistent framework. Our method utilizes a background NNLM which models generic background text together with a collection of domain-specific entities modeled as individual FSTs. Each output token is generated by a mixture of these components; the mixture weights are estimated with a separately trained neural decider. We show that NFCLM significantly outperforms NNLM by 15.8% relative in terms of Word Error Rate. NFCLM achieves similar performance as traditional NNLM and FST shallow fusion while being less prone to overbiasing and 12 times more compact, making it more suitable for on-device usage.

==> introduction.tex <==
End-to-end (E2E) models such as the neural transducers with transformer~\cite{VaswaniShazeerParmarEtAl17} or long short term memory (LSTM)~\cite{HochreiterSchmidhuber97} encoders~\cite{Graves12, GravesMohamedHinton13, RaoSakPrabhavalkar17, YehMahadeokarKalgaonkar19, ZhangLuSakEtAl20, ShiWangWuEtAl21}, attention-based encoder-decoder models~\cite{ChanJaitlyLeEtAl16, BahdanauChorowskiSerdyukEtAl16, KimHoriWatanabe17, ChiuSainathWeEtAl18, ZeyerIrieSchluterEtAl18}
%, and connectionist temporal classification (CTC)~\cite{GravesFernandezGomezEtAl06} with word- or grapheme-based output units~\cite{GravesJaitly14,SoltauLiaoSak17},
are becoming increasingly popular for automatic speech recognition (ASR).
These models are particularly attractive from the point of view of on-device ASR: since they output grapheme-based units, they do not require the use of a separate lexicon, or a compiled decoder graph to map sub-word outputs to word sequences; furthermore, their compact size and all-neural architectures allow for relatively accurate transcriptions with a small memory and computational footprint~\cite{HeSainathPrabhavalkarEtAl19, KimLeeGowdaEtAl19}.

Unlike conventional hybrid ASR systems~\cite{MorganBourlard95} -- which consist of separately trained acoustic (AM) and language model (LM) components -- end-to-end models are trained jointly on paired acoustic-text data.
If paired data are available for all domains of interest, then end-to-end models can be made more robust by training on data sampled from all domains~\cite{NarayananPrabhavalkarChiuEtAl19}.
However, in many practical situations it is unreasonable to expect that paired data are available for all domains -- either because such data collection would be prohibitively expensive, impractical, or both.
Thus, %we are presented with
two related challenges that must be addressed in the end-to-end modeling framework in order to make them suitable replacement for conventional hybrid systems: first, it must be possible to rapidly adapt an end-to-end ASR system to a new domain of interest, potentially unseen during training; second, it must be possible to correctly recognize words -- e.g., named entities -- which might occur infrequently in the training data, but might be known to be relevant during decoding.
The first of these challenges has been addressed in previous work through \emph{language model fusion}~\cite{GulcehreFirhatXuEtAl15, KannanWuNguyenEtAl18, SriramJunSatheeshEtAl17}; %by training a separate LM which can significantly improve performance on out-of-domain utterances.
%When combined with internal language model (ILM) subtraction~\cite{McDermottSakVariani19, VarianiRybachAllauzenEtAl20, MengParthasarthySunEtAl21, ZeyerMerboldtMichel21}, language model fusion can significantly improve performance on out-of-domain utterances.
the second challenge -- recognizing rare words -- has been most successfully addressed in the setting where we have a set of specific entities and the corresponding context in which they are likely to occur (e.g., the user's contact list; song playlists; etc.) through \emph{shallow fusion biasing}~\cite{ZhaoSainathRybachEtAl19,Le2021deepshallow,le21_interspeech}.
%(e.g., the user's contact list; song playlists; etc.) by biasing the decoding process using a specifically constructed finite state transducer (FST)~\cite{MohriPereiraRiley02} which encodes the relevant entities along with contextual n-grams where they are likely to be found

In this work, we focus on the problem of developing an end-to-end model which can perform well on multiple domains, where a subset of domains are only available as a set of context-free grammar (CFG) rules~\cite{HopcroftMotwaniUllman01}.
% \footnote{For example, a music domain grammar might contain the patterns \texttt{play @song} or \texttt{play @song by @artist}. \texttt{@song} and \texttt{@artist} represent non-terminals. {\color{red}See Section~\ref{sec:training} for more details.}}
This setting presents an important challenge when building speech-enabled voice assistants that must be able to support downstream spoken language understanding (SLU) systems which constantly expand coverage by serving new domains, without the need to keep re-training the E2E model.
As a solution to this challenge, we propose a \emph{Neural-FST Class Language Model (NFCLM)}, an approach that builds a factorized LM consisting of a background LM combined with separate domain-specific LMs; each word in the sentence is then generated by this mixture of LM components weighted by a separately estimated \emph{decider}.
Crucially, the proposed solution combines neural LMs~\cite{BengioDucharmeVincentEtAl03, MikolovKombrinkBurgetEtAl11} to represent \emph{general data}, and FST-based LMs to represent domain-specific substitution patterns (i.e., named entities).
%The use of FST-based LMs allows for dynamic injection of specific entities during decoding similar to their use in contextual biasing~\cite{ZhaoSainathRybachEtAl19,Le2021deepshallow,le21_interspeech,HallChoAllauzenEtAl15}.

%In this section, we provide a brief review of prior work related to the present work -- improving end-to-end ASR performance to support multiple domains, or more broadly, to better recognize words which are seen infrequently in the training data. Broadly speaking, these techniques can be divided into two categories: those that focus on retraining the end-to-end model itself, and those that focus on improving robustness during decoding through biasing, or improved LMs.


==> related_work.tex <==
%In this section, we provide a brief review of prior work related to the present work -- improving end-to-end ASR performance to support multiple domains, or more broadly, to better recognize words which are seen infrequently in the training data. Broadly speaking, these techniques can be divided into two categories: those that focus on retraining the end-to-end model itself, and those that focus on improving robustness during decoding through biasing, or improved LMs.
%Techniques for improving end-to-end ASR accuracy on rare words and diverse domains can be broadly divided into two categories: those that focus on retraining the end-to-end model, and those that focus on improving recognition through biasing, or improved LMs.
%An example of the former approach, 
%which has been explored in previous work, 
One approach to improving E2E ASR on specific domains represented as CFGs is to generate sentences from the underlying domain grammar, and then generate the corresponding acoustic sequences using a text-to-speech system (e.g.,~\cite{HeSainathPrabhavalkarEtAl19, KaritaWatanabeIwataEtAl19, RosenbergZhangRamabhadranEtAl19} \emph{inter alia}).
However, this approach is computationally expensive -- both the TTS synthesis process as well as the effort required to re-train the end-to-end-model -- which makes it harder to rapidly adapt to a new domain or support substitution patterns which are only available at inference time.
Therefore, in this work we focus on improving recognition of a pre-trained ASR system by improving the LM used during decoding.

The simplest approach to building LMs which cover multiple domains -- some of which are represented as CFGs -- is to generate domain-specific data by substituting non-terminal symbols~\cite{GalescuRinggerAllen98, WangMahajanHuang00}.
This data can then be pooled together with the ``background" text to train a single LM with wider coverage.
While this solution is simple to implement, it is only applicable in cases where all of the non-terminal substitution patterns are known at training time, or if they form a closed set (e.g., numeric patterns, or dates); extending this solution to the case where some of the patterns are only available during inference is not trivial for neural LMs.

An alternative approach -- employed extensively in hybrid ASR systems~\cite{MorganBourlard95} -- consists of the use of class-based non-terminals in the decoder graph to represent classes of interest (e.g., contact names, songs, artists, etc.); these can then be replaced on-the-fly using separate FSTs which can be compiled and personalized for each user~\cite{SchalkwykHetheringtonStory03, DixonHoriKashioka12, AleksicAllauzenElsonEtAl15}.
However, end-to-end models are typically decoded without a separate N-gram LM or decoder graph.
Instead, the common solution in this case involves shallow-fusion contextual biasing~\cite{ZhaoSainathRybachEtAl19, HaynorAleksic20,Le2021deepshallow, le21_interspeech} -- i.e., the application of finite state transducers (FST)s~\cite{MohriPereiraRiley02} representing various entities of interest in particular contexts which can be applied during decoding for salient entities.
The FST-based biasing techniques has two disadvantages: it is somewhat challenging to set the weights in the biasing FST -- typically, these are hand-tuned on a development set; and, there is a danger of overbiasing phrases if the biasing weights are set to inappropriate values, although this can be mitigated somewhat by only allowing the biasing to be applied in specific contexts~\cite{HeSainathPrabhavalkarEtAl19}. Attempts at relieving the issue use the ASR model's output to decide when to trigger \cite{appleclasslms} but this means that the LM is tied to the recognizer instead of being stand-alone.

Our proposed approach is to build a factorized LM which can cover all domains of interest, and use this LM in shallow fusion with internal LM subtraction~\cite{VarianiRybachAllauzenEtAl20} during decoding.
We propose to train a separate LM for the ``background" text data -- which is intended to have broad coverage -- as well as multiple domain specific LMs which have narrower coverage, similar to previous work on mixture-of-expert LMs~\cite{ShazeerMirhoseiniMaziarzEtAl17, IrieKumarNirschlEtAl18}. 
These various component LMs are combined through a separate \emph{decider} network which generates the next word from the mixture of component LMs, thus interpolating them.
In particular, the domain specific LMs are represented using FSTs, as in shallow-fusion biasing~\cite{ZhaoSainathRybachEtAl19}, however, these are integrated in a purely probabilistic model to generate scores that can be interpreted as probabilities, without the need for hand-tuning of biasing weights.
Leveraging FSTs to represent the domain-specific entities makes it easier to dynamically add specific entities during inference.
{\color{red} https://www.overleaf.com/project/612f9ab891a5163eb1dd2c07#
Finally, we note that the proposed techniques are complementary with standard shallow-fusion contextual biasing approaches~\cite{ZhaoSainathRybachEtAl19,Le2021deepshallow,le21_interspeech}; indeed, as can be seen in Section~\ref{sec:results}, we obtain our best results when the proposed LM models are evaluated with shallow-fusion biasing.
}

\begin{figure*}
\include{tikz_fst}
\caption{NFCLM's expanded dynamic FST after consuming the output symbol sequence $\mathbf{h^w} = \{\_play, \_ros, ie, \_by, \_browne\}$. The decider histories $\mathbf{h^\text{decider}}$ left inside the beam after each extension are displayed on the state label. Here we assume that there are two classes, $@song$ (red) and $@artist$ (green), in addition to the background states (blue). These non-background classes are represented by the component FSTs shown in Fig.~\ref{fig:bias_fst}. At the last stage, two paths are dropped from the beam (gray). As an illustration, we have the probabilities: $P_1=P_d(@bg|\mathbf{h^\text{mixed}}).P_{@bg}(\_play|\mathbf{h^w})$,
$P_2=P_d(@song|\mathbf{h^\text{mixed}}).FST_{@song}(0 \rightarrow 1)$,
$P_3=FST_{@song}(1 \rightarrow 2)$,
$P_4=Final_{@song}(2).P_d(@bg|\mathbf{h^\text{mixed}}).P_{@bg}(\_by|\mathbf{h^w})$, and
$P_5=P_d(@artist|\mathbf{h^\text{mixed}}).FST_{@artist}(0 \rightarrow 1)$.
}
\label{fig:dfst}
\end{figure*}


==> state_table.tex <==

\begin{tabular}{|l|l|l|l|l|l|}
\hline
 & Decider history & BG history &  & Label \\
\hline
1 &  &  & - & \texttt{<s>} \\
\hline
\color{orange}
2 & \texttt{<s>} & \texttt{<s>} & - & \texttt{\_play} \\
\hline
\color{blue}
3 & \texttt{<s> \_play} & \texttt{<s> \_play} & 0 & \texttt{@artist} \\
\hline
\color{orange}
4 & \texttt{<s> \_play} & \texttt{<s> \_play} & - & \texttt{\_rosa} \\
\hline
\color{orange}
5 & \texttt{<s> \_play} & \texttt{<s> \_play} & - & \texttt{\_pop} \\
\hline
\color{blue}
6 & \texttt{<s> \_play} & \texttt{<s> \_play} & 1 & \texttt{\_jay} \\
  & \texttt{@artist} &  &  &  \\
\hline
\color{blue}
7 & \texttt{<s> \_play} & \texttt{<s> \_play} & 3 & \texttt{\_bach} \\
  & \texttt{@artist} & & & \\
\hline
\color{orange}
8 & \texttt{<s> \_play} & \texttt{<s> \_play} & - & \texttt{lie} \\
  & \texttt{\_rosa} & \texttt{\_rosa} & &  \\
\hline
\color{blue}
9 & \texttt{<s> \_play} & \texttt{<s> \_play} & 2 & \texttt{z} \\
  & \texttt{@artist} & \texttt{\_jay} & & \\
\hline

\end{tabular}


